Predicting Game Engagement and Difficulty Using AI Players

This paper presents a novel approach to automated playtesting for the prediction of human player behavior and experience. It has previously been demonstrated that Deep Reinforcement Learning (DRL) game-playing agents can predict both game difficulty and player engagement, operationalized as average pass and churn rates. We improve this approach by enhancing DRL with Monte Carlo Tree Search (MCTS). We also motivate an enhanced selection strategy for predictor features, based on the observation that an AI agent's best-case performance can yield stronger correlations with human data than the agent's average performance. Both additions consistently improve the prediction accuracy, and the DRL-enhanced MCTS outperforms both DRL and vanilla MCTS in the hardest levels. We conclude that player modelling via automated playtesting can benefit from combining DRL and MCTS. Moreover, it can be worthwhile to investigate a subset of repeated best AI agent runs, if AI gameplay does not yield good predictions on average.

==> ModifiedMCTSAlgorithm.tex <==
\begin{algorithm}
	\caption{NN Modified MCTS algorithm}
	\begin{algorithmic}[1]
        \Function{MCTS}{$node$}
            \While{simulation budget is available}
                \For{number of parallel environments}
                    \State $node \gets $\Call{Select}{$ $}
                    \State $(child, score) \gets $\Call{Expand}{$node$}
                    \State \Call{BackPropagate}{$child, score$}
                \EndFor
                %\State \Call{BackPropagate}{$child, score$}
             \EndWhile
        \EndFunction
	    \Function{Select}{$ $}
            \While{node is not completely expanded \textbf{and} node is not terminal}
                \State $node \gets $\Call{BestChild}{$node$}
            \EndWhile
            \State \Return $node$
        \EndFunction
        \Function{BestChild}{$node$}
    	    \State \Return $\argmax_{ch \in node.children} ch.r+\gamma \frac{ch.V}{ch.N}+c\sqrt{\frac{\log{node.N+node.O}}{ch.N+ch.O}}$ \label{line:updated-ucb}
            %\State \[\Return \argmax_{ch \in node.children} ch.r+\gamma %\frac{ch.V}{ch.N}+c\sqrt{\frac{\log{(node.N+node.O)}}{ch.N+ch.O}}\] \label{line:updated-ucb}
        \EndFunction
        \Function{Expand}{$node$}
            \State Select action $a \in$ node's unexplored children based on $\pi^{RL}(node.s)$
            \State $s', r \gets f(node.s, a)$
            \State $node.children.add(child)$ and $child.parent \gets node$
            \State $child.s \gets s'$
            \State $child.a \gets a$
            \State $child.r \gets r$ \label{line:store_imr}
            \State $child.O \gets child.O+1$ \Comment{O is an auxiliary variable for parallelization} %\Comment{\makecell{auxiliary variable for \\parallelization}}
            \While{node is not null}\label{line:increasesO}
                \State $node.O \gets node.O+1$
                \State $node \gets node.parent$ \label{line:increasesO-2}
            \EndWhile
            \State \Return ($child,$ \Call{Rollout}{$child.s$})
        \EndFunction
        \Function{Rollout}{$s$}
            \State $score \gets 0$
            \State $t \gets 0$
            %\While{s \textbf{not} terminal}
            \While{s \textbf{not} terminal \textbf{and} $t < time horizon$}
                \State $a \gets \pi^{RL}(s)$
                \State $s', r \gets f(s, a)$
                \State $s \gets s'$
                \State $t \gets t+1$
                \State $score \gets score + \gamma^{t} r$ \label{line:discounted-reward}
            \EndWhile
            \State \Return score
        \EndFunction
        \Function{BackPropagate}{$node, score$}
            %\State $r \gets 0$
            \State $v \gets score$
            \While{node is not null}
                %\State $node.V \gets node.V + v + r$
                \State $node.V \gets node.V + v$ \label{line:storeV}
                \State $node.N \gets node.N + 1$
                \State $node.O \gets node.O - 1$ \label{line:decreaseO}
                %\State $r \gets node.r$
                %\State $v \gets \gamma (node.V/node.N)$
                \State $v \gets node.r + \gamma (node.V/node.N) $ \label{line:discounted-baclpropagation}
                \State $node \gets node.parent$
            \EndWhile
        \EndFunction
	\end{algorithmic}
	\label{algo:nn-modified-mcts}
\end{algorithm}

==> method_1.tex <==
%!TEX root = main.tex
\section{Method}\label{sec:method}
This paper utilizes similar high-level population simulation, reward function formulation, and DRL agents trained for each level as Roohi et al. \cite{roohi2020predicting}. What is new is augmenting the DRL game play with MCTS, and improving the features extracted from the AI gameplay data. The changes are motivated by how Roohi et al. \cite{roohi2020predicting} observed that 1) churn predictions were more accurate if using ground truth human pass rate data instead of simulated predictions, and 2) the simulated pass rate predictions were particularly inaccurate for the most difficult levels. To improve the predictions, it was logical to try to employ MCTS in addition to DRL, as the combination has been highly successful in playing very challenging games like StarCraft and Go \cite{silver2016mastering, vinyals2019alphastar}. Motivated by Kristensen et al. \cite{kristensen2020estimating} and the high variability of the DRL agent's performance, we also hypothesized that the difficulty of the hardest levels would be better predicted by the agent's best case performance rather than average performance. To implement this, we employed multiple attempts per level and only utilized the data from the most successful attempts. 


\subsection{Monte-Carlo tree search}
MCTS is an alternative to DRL in solving MDP:s. Instead of training a neural network, MCTS decides the approximately optimal action by building a tree of possible future game states and rewards, each tree node corresponding to the state resulting from an explored action. The root of the tree corresponds to the current state. More specifically, MCTS iterates over 4 steps \cite{yannakakis2018artificial}:
\begin{itemize}
    \item Select: traverse down the tree until at a node with non-explored actions. Children are selected using the Upper Confidence Bound fot Trees (UCT) formula:  
    \begin{equation}\label{eq:ucb}
        \argmax_{ch \in node.children} \frac{ch.V}{ch.N}+c\sqrt{\frac{\ln{node.N}}{ch.N}},
    \end{equation}
    where $ch$ denotes a child considered, $V$ denotes value, and $N$ denotes the number of visits so far. The $c$ parameter adjusts the exploration-exploitation tradeoff and is usually set to \textcolor{blue}{$\sqrt{2}$ \cite{kocsis2006bandit}, which is the value that have been used in our experiments.} \todo{cite a textbook source for the theoretically optimal c, and explain what value we use}.
    \item Expand: the selected node is expanded by taking a random non-explored action and a new node is added as a child of the selected node. 
    \item Rollout simulation: run the game forward from the added child with random actions until at a terminal state (level passed or out of moves) \textcolor{blue}{I used time horizon of 10, so until at the terminal state or 10 moves}, updating the value of the added child as $ch.V=\sum_t \gamma^t r_t$, where $\gamma$ is a discount factor, $t$ is simulation timestep and $r_t$ is the reward received at step $t$. 
    \item Backpropagate: the simulation results are propagated toward the root, updating the value of each node as \todo{add update equation here. This way, we can remove Algorithm 1, as all the terms discussed are defined precisely enough without it, including $r$ .} \textcolor{blue}{For the Vanilla MCTS, I did not use discounted backpropagation and increased the value of the new node and its ancestors by the rollout return, It is not same as having the $\gamma=1.0$.}
    \begin{equation}
    N_{s_{t-1}} \gets N_{s_{t-1}} + 1,\quad V_{s_{t-1}} \gets V_{s_{t-1}} + r_{t-1} + \gamma \frac{V_{s_t}}{N_{s_t}}
    \end{equation}
    \textcolor{blue}{The backpropagation update that I have used righ now is like equation 2, however it should be like equation 3. If the update was like equation 3, we could say that the Vanilla MCTS update is in a discounted way with $\gamma=1.0$. Maybe, we have to re-run the experiments with this new update rule and a smaller gamma instead of performing greedy.}
    \begin{equation}
    N_{s_{t-1}} \gets N_{s_{t-1}} + 1,\quad V'_{s_{t-1}} \gets r_{t-1} + \gamma V'_{s_t},\quad V_{s_{t-1}} \gets V_{s_{t-1}} + V'_{s_{t-1}}
    \end{equation}
\end{itemize}

\subsubsection{Tested MCTS Variants}
We first tested vanilla MCTS without modifications, but this required prohibitively many moves to pass a level and did not produce better results than in Roohi et al. \cite{roohi2020predicting}. To address the problem, we developed and tested the following modifications:% \todo{Rename "Modified MCTS" to "Greedy MCTS", as that's more descriptive. Also: could similar results be simply achieved by using a smaller gamma? The modification is not super well motivated if you don't first run the MCTS with different gamma to ensure that decreasing gamma doesn't improve results just as much. }

\begin{itemize}
    \item NN MCTS: Instead of random actions, this version samples the rollout simulation actions from a DRL game playing policy trained similar to Roohi et al. \cite{roohi2020predicting}. This is a generally applicable technique inspired by AlphaGo \cite{silver2016mastering}. Because of the less random rollout actions, the backpropagated values have less variance, which results in better choices for the selected and expanded nodes. An alternative view is that this allows MCTS to improve on the results of an imperfect DRL agent. We have found this particularly effective in increasing the AI pass rates of very hard levels. 
    \item Greedy MCTS: This modification uses a slightly modified UCT formula to give more weight to the immediate reward $r$ of each action: 
    \begin{equation}\label{eq:updated_ucb}
        \argmax_{ch \in node.children} ch.r+\gamma \frac{ch.V}{ch.N}+c\sqrt{\frac{\ln{node.N}}{ch.N}}.
    \end{equation}
    This is a game-specific modification that exploits how the immediate rewards are predictive of longer term AI success, in our case. 
    \item NN-Greedy MCTS: this version combines both modifications. 
\end{itemize}

\subsubsection{Implementation Details}
Time horizon of 10 and discount factor $\gamma=0.9$ was used. Discounting was used because the game is non-deterministic and rewards far away in the future have high variance. The discounting helps to reduce the variance, especially as our simulation budget is limited. A simulation budget of 200 was assigned to each state, resulting in a tree depth of approximately 4. Each MCTS run used 16 parallel instances of the game. For each level, MCTS agent was run for 20 times, which took about 10 hours per level, and \todo{1680} \textcolor{blue}{I don't know the exact number} for all the \todo{168} levels we had the ground truth human data for.


To reduce the amount of simulation needed, we assume that the game dynamics are deterministic, i.e., the same action from the same current state always results in the same next state. This allows us to cache the rollout states and actions and reuse them in the tree expansion. \textcolor{blue}{I didn't save the rollout states. I just assumed that expanding a node always results into the same next sate.} Assuming determinism also allows reusing the subtree below the selected action when moving to the next game state and restarting the tree search.  
%We augmented the Unity ML-Agent framework \cite{juliani1809unity} by the MCTS algorithm so we could run it in parallel. According to \cite{liu2018watch}, we added an auxiliary variable to each node for better exploration in the face of in-progress simulations due to parallelization. When a node is expanded, the value of this variable in that node and all of its ancestors are increased (lines \ref{line:increasesO}-\ref{line:increasesO-2}). After all the parallel simulations were completed, backpropagation is called. During backpropagation these increased values are reduced again (line \ref{line:decreaseO}). In addition, The UCB formula is altered to the line \ref{line:updated-ucb} of the algorithm  \ref{algo:nn-modified-mcts}.

Table \ref{tab:mctsVersions} shows the average performance of four MCTS versions over 20 runs on the five hardest levels of the dataset. Since NN-Greedy MCTS has the best performance, it was selected to run on all of the levels. \todo{does vanilla MCTS use $\gamma=0.9$ or $\gamma=1.0$?} \textcolor{blue}{for the rollout return, I used $\gamma=0.9$ for all the MCTS variants. However, For the Vanilla MCTS, I did not use discounting backpropagation and increased the value of the new node and its ancestors by the rollout return, It is not same as having the $\gamma=1.0$.} %For the rest of paper, NN-Greedy MCTS will be mentioned by MCTS for convenience.
%\input{ModifiedMCTSAlgorithm}
\input{mctsVersionsTab}


\subsection{Feature selection}
%\todo{Use the NN-Greedy MCTS term consistently hereafter, and DRL for the DRL agent without MCTS. When talking about the versions with enhanced feature selection, use NN-Greedy MCTS-F and DRL-F.}

In this section, we explain our feature selection, which varies from those used by Roohi et al. \cite{roohi2020predicting}. Inspired by \cite{kristensen2020estimating}, We computed the Spearman correlation between the average of agent's performance in different portions of its best runs with the human players pass rates. The portions that produced the highest correlation was selected to calculate the input features. Overall, for each game level, the trained DRL agent was run for 1000 times and its statistics were recorded. The games with the highest moves left after passing the level were considered as the best runs.

Figure \ref{fig:rl_correletion} indicates that although average of moves left out of 4x moves ratio and cleared goals percentage have lower correlation with human players' pass rates when we use large portion of runs, pass rate and average used moves ratio correlation with human players pass rates is higher when we use all the collected data. Thus, average of moves left out of 4x moves ratio and cleared goals percentage were calculated by 15\% and 5\% of the best agent's runs, respectively. However we used all of the runs for computing the pass rate and average used moves ratio. In total, these 4 features are defined as the high-correlated input features.
\begin{figure}[hbt!]
	\centering
	\includegraphics[width=0.99\textwidth]{figures/rl_correletion.png}
	\caption{Correlation between RL statistics and the players' pass rates.}	
	\label{fig:rl_correletion}
\end{figure}

==> mseTab_old.tex <==
\begin{table}[hbt!]
\centering
\caption{Mean and standard deviation of Pass and churn rate MSEs over 25 runs of 5-fold cross validation, calculated by baseline and extended models with different input features. DRL-F features are computed by the portion of the best DRL runs that shows higher correlation with the human players pass rates. NN-Greedy MCTS uses 16 input features same as the Roohi et al DRL agent. NN-greedy MCTS Mean contains 3 features including average passes, average moves left ratio, and average cleared goals percentage. NN-Greedy MCTS Mean-F features are formed by combination of 4 features from DRL-F and the 3 features from NN-Greedy MCTS Mean.}~\label{tab:mseTab}
\begin{tabular}{|c|c|c|}
\hline
Method & Pass rate MSE & Churn rate MSE \\ \hline
\makecell{Baseline Roohi et al. \\ DRL} & \makecell{$\mu=0.01890$ \\ $\sigma=0.00514$}            & \makecell{$\mu=0.00014$ \\ $\sigma=0.00003$} \\ \hline
\makecell{Our Baseline \\ DRL-F} & \makecell{$\mu=0.01738$ \\ $\sigma=0.00367$}            & \makecell{$\mu=0.00012$ \\ $\sigma=0.00003$} \\ \hline
\makecell{Our Baseline \\ NN-Greedy MCST} & \makecell{$\mu=0.02040$ \\ $\sigma=0.00370$}            & \makecell{$\mu=0.00013$ \\ $\sigma=0.00003$} \\ \hline
\makecell{Our Baseline \\ NN-Greedy MCTS Mean} & \makecell{$\mu=0.01919$ \\ $\sigma=0.00305$}            & \makecell{$\mu=0.00012$ \\ $\sigma=0.00003$} \\ \hline
\makecell{Our Baseline \\ NN-Greedy MCTS Mean-F} & \makecell{$\mu=0.01436$ \\ $\sigma=0.00207$}            & \makecell{$\mu=0.00012$ \\ $\sigma=0.00003$} \\ \hline
\makecell{Extended Roohi et al. \\ DRL} & \makecell{$\mu=0.01953$ \\ $\sigma=0.00482$}            & \makecell{$\mu=0.00008$ \\ $\sigma=0.00002$} \\ \hline
\makecell{Our Extended \\ DRL-F} & \makecell{$\mu=0.01729$ \\ $\sigma=0.00479$}        & \makecell{$\mu=\textbf{0.00007}$ \\ $\sigma=\textbf{0.00002}$} \\ \hline
\makecell{Our Extended \\ NN-Greedy MCTS} & \makecell{$\mu=0.02048$ \\ $\sigma=0.00405$}            & \makecell{$\mu=0.00008$ \\ $\sigma=0.00002$} \\ \hline
\makecell{Our Extended \\ NN-Greedy MCTS Mean} & \makecell{$\mu=0.01925$ \\ $\sigma=0.00369$}            & \makecell{$\mu=0.00008$ \\ $\sigma=0.00002$} \\ \hline
\makecell{Our Extended \\NN-Greedy MCTS Mean-F} & \makecell{$\mu=\textbf{0.01410}$ \\ $\sigma=\textbf{0.00224}$}        & \makecell{$\mu=\textbf{0.00007}$ \\ $\sigma=\textbf{0.00002}$} \\ \hline
\end{tabular}
\end{table}

